Adversarial Perturbations Against Deep Neural Networks for Malware Classification

Deep neural networks, like many other machine learning models, have recently been shown to lack robustness against adversarially crafted inputs. These inputs are derived from regular inputs by minor yet carefully selected perturbations that deceive machine learning models into desired misclassifications. Existing work in this emerging field was largely specific to the domain of image classification, since the high-entropy of images can be conveniently manipulated without changing the images' overall visual appearance. Yet, it remains unclear how such attacks translate to more security-sensitive applications such as malware detection - which may pose significant challenges in sample generation and arguably grave consequences for failure. In this paper, we show how to construct highly-effective adversarial sample crafting attacks for neural networks used as malware classifiers. The application domain of malware classification introduces additional constraints in the adversarial sample crafting problem when compared to the computer vision domain: (i) continuous, differentiable input domains are replaced by discrete, often binary inputs; and (ii) the loose condition of leaving visual appearance unchanged is replaced by requiring equivalent functional behavior. We demonstrate the feasibility of these attacks on many different instances of malware classifiers that we trained using the DREBIN Android malware data set. We furthermore evaluate to which extent potential defensive mechanisms against adversarial crafting can be leveraged to the setting of malware classification. While feature reduction did not prove to have a positive impact, distillation and re-training on adversarially crafted samples show promising results.

==> accuracy_table.tex <==
%! TEX root = main.tex

\begin{table*}
\centering
\scriptsize
\begin{tabular}{l | c | c | c| c| c}
Restriction & Shape & Malware Ratio & Accuracy/\% & FNR/\% & FPR/\% \\ \hline
manifestonly  	& [100, 100] 	 & 0.3 	 & 96.8 	 & 11.655 	 & 2.778 \\
manifestonly  	& [100, 100] 	 & 0.4 	 & 96.242 	 & 12.896 	 & 3.305 \\
manifestonly  	& [100, 100] 	 & 0.5 	 & 95.408 	 & 10.594 	 & 4.28 \\
manifestonly  	& [100, 200] 	 & 0.3 	 & 97.277 	 & 12.68 	 & 2.233 \\
manifestonly  	& [100, 200] 	 & 0.4 	 & 97.588 	 & 14.658 	 & 1.819 \\
manifestonly  	& [100, 200] 	 & 0.5 	 & 95.01 	 & 10.324 	 & 4.709 \\
manifestonly  	& [200, 100] 	 & 0.3 	 & 96.484 	 & 9.73 	 & 3.195 \\
manifestonly  	& [200, 100] 	 & 0.4 	 & 96.13 	 & 11.529 	 & 3.484 \\
manifestonly  	& [200, 100] 	 & 0.5 	 & 96.648 	 & 12.14 	 & 2.915 \\
manifestonly  	& [200, 200, 200, 200] 	 & 0.3 	 & 98.32 	 & 22.896 	 & 0.683 \\
manifestonly  	& [200, 200, 200, 200] 	 & 0.4 	 & 98.144 	 & 25.36 	 & 0.756 \\
manifestonly  	& [200, 200, 200, 200] 	 & 0.5 	 & 97.683 	 & 20.27 	 & 1.467 \\
manifestonly  	& [200, 200] 	 & 0.3 	 & 98.497 	 & 15.971 	 & 0.831 \\
manifestonly  	& [200, 200] 	 & 0.4 	 & 95.145 	 & 9.838 	 & 4.61 \\
manifestonly  	& [200, 200] 	 & 0.5 	 & 95.101 	 & 8.957 	 & 4.696 \\
manifestonly  	& [200, 400] 	 & 0.3 	 & 98.207 	 & 14.91 	 & 1.161 \\
manifestonly  	& [200, 400] 	 & 0.4 	 & 95.88 	 & 9.874 	 & 3.819 \\
manifestonly  	& [200, 400] 	 & 0.5 	 & 94.892 	 & 9.568 	 & 4.866 \\
manifestonly  	& [300, 200] 	 & 0.3 	 & 97.602 	 & 12.212 	 & 1.915 \\
manifestonly  	& [300, 200] 	 & 0.4 	 & 96.741 	 & 11.781 	 & 2.834 \\
manifestonly  	& [300, 200] 	 & 0.5 	 & 95.349 	 & 9.982 	 & 4.37 \\
manifestonly  	& [400, 200] 	 & 0.3 	 & 96.579 	 & 10.144 	 & 3.076 \\
manifestonly  	& [400, 200] 	 & 0.4 	 & 96.872 	 & 12.86 	 & 2.649 \\
manifestonly  	& [400, 200] 	 & 0.5 	 & 95.842 	 & 9.496 	 & 3.876 \\
	 	& [100, 200] 	 & 0.4 	 & 97.43 	 & 8.345 	 & 2.269 \\
	 	& [10, 10] 	 & 0.3 	 & 97.592 	 & 16.367 	 & 1.738 \\
	 	& [10, 10] 	 & 0.4 	 & 94.853 	 & 9.676 	 & 4.901 \\
	 	& [10, 10] 	 & 0.5 	 & 94.752 	 & 7.338 	 & 5.112 \\
	 	& [10, 200] 	 & 0.3 	 & 97.529 	 & 11.205 	 & 2.036 \\
	 	& [10, 200] 	 & 0.4 	 & 96.143 	 & 8.669 	 & 3.599 \\
	 	& [10, 200] 	 & 0.5 	 & 94.255 	 & 5.719 	 & 5.705 \\
	 	& [200, 100] 	 & 0.4 	 & 97.316 	 & 9.227 	 & 2.348 \\
	 	& [200, 100] 	 & 0.5 	 & 96.345 	 & 6.655 	 & 3.479 \\
	 	& [200, 10] 	 & 0.3 	 & 95.627 	 & 15.252 	 & 3.863 \\
	 	& [200, 10] 	 & 0.4 	 & 93.945 	 & 10.809 	 & 5.821 \\
	 	& [200, 10] 	 & 0.5 	 & 92.966 	 & 8.957 	 & 6.927 \\
	 	& [200, 200, 200, 200] 	 & 0.4 	 & 97.417 	 & 13.076 	 & 2.07 \\
	 	& [200, 200, 200, 200] 	 & 0.5 	 & 97.5 	 & 12.374 	 & 2.014 \\
	 	& [200, 200, 200] 	 & 0.1 	 & 98.911 	 & 17.482 	 & 0.309 \\
	 	& [200, 200, 200] 	 & 0.4 	 & 97.685 	 & 10.342 	 & 1.912 \\
	 	& [200, 200] 	 & 0.1 	 & 98.915 	 & 17.176 	 & 0.319 \\
	 	& [200, 200] 	 & 0.2 	 & 98.347 	 & 8.741 	 & 1.293 \\
	 	& [200, 200] 	 & 0.3 	 & 97.669 	 & 7.5 	 & 2.057 \\
	 	& [200, 200] 	 & 0.4 	 & 97.492 	 & 7.014 	 & 2.264 \\
	 	& [200, 200] 	 & 0.5 	 & 96.496 	 & 6.871 	 & 3.311 \\
	 	& [200, 300] 	 & 0.3 	 & 98.352 	 & 9.586 	 & 1.249 \\
	 	& [200, 300] 	 & 0.4 	 & 97.618 	 & 8.741 	 & 2.054 \\
	 	& [200, 50] 	 & 0.3 	 & 96.889 	 & 6.367 	 & 2.944 \\
	 	& [200, 50] 	 & 0.4 	 & 95.867 	 & 5.36 	 & 4.057 \\
	 	& [200, 50] 	 & 0.5 	 & 93.933 	 & 4.55 	 & 6.115 \\
	 	& [200] 	 & 0.4 	 & 97.832 	 & 8.058 	 & 1.861 \\
	 	& [200] 	 & 0.5 	 & 95.845 	 & 5.414 	 & 4.057 \\
	 	& [300, 200] 	 & 0.2 	 & 98.127 	 & 9.335 	 & 1.496 \\
	 	& [300, 200] 	 & 0.4 	 & 97.285 	 & 8.058 	 & 2.433 \\
	 	& [50, 200] 	 & 0.3 	 & 97.583 	 & 17.302 	 & 1.705 \\
	 	& [50, 200] 	 & 0.4 	 & 97.351 	 & 10.144 	 & 2.292 \\
	 	& [50, 200] 	 & 0.5 	 & 95.654 	 & 6.007 	 & 4.251 \\
	 	& [50, 50] 	 & 0.3 	 & 96.569 	 & 12.572 	 & 2.978 \\
	 	& [50, 50] 	 & 0.4 	 & 96.789 	 & 13.076 	 & 2.725 \\
	 	& [50, 50] 	 & 0.5 	 & 93.824 	 & 6.763 	 & 6.108 \\
onlyfreq 1  	& [200, 200] 	 & 0.3 	 & 97.673 	 & 7.5 	 & 2.053 \\
onlyfreq 1  	& [200, 200] 	 & 0.4 	 & 96.538 	 & 7.518 	 & 3.238 \\
onlyfreq 1  	& [200, 200] 	 & 0.5 	 & 97.258 	 & 7.446 	 & 2.489 \\
onlyfreq 2  	& [200, 200] 	 & 0.3 	 & 97.957 	 & 7.716 	 & 1.746 \\
onlyfreq 2  	& [200, 200] 	 & 0.4 	 & 97.89 	 & 9.388 	 & 1.741 \\
onlyfreq 2  	& [200, 200] 	 & 0.5 	 & 95.009 	 & 5.126 	 & 4.944 \\
onlyfreq 3  	& [200, 200] 	 & 0.3 	 & 98.223 	 & 8.561 	 & 1.43 \\
onlyfreq 3  	& [200, 200] 	 & 0.4 	 & 97.51 	 & 8.129 	 & 2.194 \\
onlyfreq 3  	& [200, 200] 	 & 0.5 	 & 96.565 	 & 5.719 	 & 3.29 \\
onlyfreq 4  	& [200, 200] 	 & 0.3 	 & 97.112 	 & 7.428 	 & 2.642 \\
onlyfreq 4  	& [200, 200] 	 & 0.4 	 & 97.497 	 & 8.957 	 & 2.171 \\
onlyfreq 4  	& [200, 200] 	 & 0.5 	 & 96.468 	 & 7.14 	 & 3.328 \\
onlysmall 1  	& [200, 200] 	 & 0.3 	 & 97.848 	 & 10.594 	 & 1.73 \\
onlysmall 1  	& [200, 200] 	 & 0.4 	 & 97.432 	 & 13.147 	 & 2.05 \\
onlysmall 1  	& [200, 200] 	 & 0.5 	 & 96.51 	 & 8.867 	 & 3.206 \\
onlysmall 2  	& [200, 200] 	 & 0.3 	 & 97.947 	 & 12.626 	 & 1.535 \\
onlysmall 2  	& [200, 200] 	 & 0.4 	 & 96.821 	 & 10.468 	 & 2.809 \\
onlysmall 2  	& [200, 200] 	 & 0.5 	 & 95.455 	 & 9.281 	 & 4.29 \\
onlysmall 3  	& [200, 200] 	 & 0.3 	 & 97.73 	 & 14.622 	 & 1.672 \\
onlysmall 3  	& [200, 200] 	 & 0.5 	 & 95.801 	 & 11.223 	 & 3.841 \\
onlysmall 4  	& [200, 200] 	 & 0.4 	 & 96.89 	 & 15.701 	 & 2.501 \\
onlysmall 5  	& [200, 200] 	 & 0.4 	 & 96.915 	 & 14.982 	 & 2.508 \\


\end{tabular}
\caption{Classification Performance of different network shapes under various feature selection restrictions.}\label{table:restricted_classifier}
\end{table*}

==> defensive_mechanisms.tex <==
%!TEX root = main.tex
%\cm{Reduce overall exposition for this section an move description of methods into their own subsections}

Considering the very huge number of features, an assumption could be that it is possible to easily craft adversarial samples since there are that many features. We will thus give a brief an short example why this could be the case. Consider a feature, that is only used by one benign app, and which could possibly be used to change the classification. 

We thus propose several approaches to do feature selection and thus restrict the set of features available for the classifier and thus also for adversarial crafting. As a start, we use some simple strategies, as just droppping large classes of the features or features that are seldomly used. 

Then we will investigate the influence of classical feature selection by using mutual information. Afterwards, we have a look at other, already tested method such as distillation or retraining on adversarial samples.

%We used the following feature selection approaches:
%\begin{itemize}
%\item restricting to manifest only features,
%\item restricting to features used in more than k Apps,
%\item removing the k biggest feature classes
%\item Using Mutual information, as in Dahl et al.\cite{DBLP:conf/icassp/DahlSDY13}
%\end{itemize} 
%The first one means that we only train the classifier on features that we can actually alter, e.g. features that appear in the manifest as in table (REF). In the second case, we only consider features that appear in several apps, to avoid that we train on features that are indicators for only k Apps.
%The third one drops the k biggest fature classes. Having a look at table~\ref{table:feature_classes}, we observe that Components and Network Addresses are very big feature classes, each on its own much bigger than all other combined. Using this selection mechanism, we drop the biggest feature classes.
%Finally we also use Mutual information as a selection criterion. The mutual information $I(X;Y)$ is the reduction of the uncertainty of $X$ due to the knowledge of $Y$\cite{DBLP:books/daglib/0016881}. Having computed the mutual information of each feature and the class,  we pick the k highest valued features and use them for training. 

==> malware_evasion.tex <==
%!TEX root = main.tex
\section{Malware Evasion for Android Apps}\label{section:malware_evasion}

\subsection{Features}
The DREBIN dataset introduced by Arp et al.~\cite{arp2014drebin} contains features describing malware on Android. It consists of 5,560 malicious applications and 123,453 benign ones. The features can be divided into ten groups, among them activities, permissions, urls, service providers, intents, calls and api-calls. The total number of instances in this classes is 545333. All the features are binary, where a one indicates the feature is present.

Even having such a large dataset, by using online learning we were able to train a deep neural network without applying feature selection. This allows us to consider all features when crafting an adversarial sample.
%\begin{itemize}
%\item around $500,000$ features in $9$ feature types
%\item we did not do any feature selection but trained on all available features
%\end{itemize}

\subsection{Model Training}
\begin{itemize}
\item describe the models that we used to classify
\item quantify training/validation and test scores of the different models, also compared with previous results
\end{itemize}

==> misclassification_table.tex <==
%!TEX root = main.tex
\begin{table*}
\centering
\scriptsize
\begin{tabular}{l | c | c |c |c |c}
Restriction & Model Shape & Malware Ratio & MissRate & Avg. Distortion & Total Samples\\ \hline
manifestonly  	& [100, 100] 	& 0.3 	& 0.944 	& 8.662 	& 5560.0 \\
manifestonly  	& [100, 100] 	& 0.4 	& 0.89 	& 9.661 	& 5560.0 \\
manifestonly  	& [100, 100] 	& 0.5 	& 0.929 	& 8.419 	& 5560.0 \\
manifestonly  	& [100, 200] 	& 0.3 	& 0.935 	& 7.913 	& 5560.0 \\
manifestonly  	& [100, 200] 	& 0.4 	& 0.969 	& 7.362 	& 5560.0 \\
manifestonly  	& [100, 200] 	& 0.5 	& 0.898 	& 9.198 	& 5560.0 \\
manifestonly  	& [200, 100] 	& 0.3 	& 0.937 	& 8.942 	& 5560.0 \\
manifestonly  	& [200, 100] 	& 0.4 	& 0.988 	& 8.316 	& 5560.0 \\
manifestonly  	& [200, 100] 	& 0.5 	& 0.959 	& 6.306 	& 5560.0 \\
manifestonly  	& [200, 200, 200, 200] 	& 0.3 	& 0.988 	& 6.887 	& 5560.0 \\
manifestonly  	& [200, 200, 200, 200] 	& 0.4 	& 0.979 	& 6.623 	& 5560.0 \\
manifestonly  	& [200, 200, 200, 200] 	& 0.5 	& 0.987 	& 6.288 	& 5560.0 \\
manifestonly  	& [200, 400] 	& 0.3 	& 0.986 	& 7.358 	& 5560.0 \\
manifestonly  	& [200, 400] 	& 0.4 	& 0.957 	& 8.985 	& 5560.0 \\
manifestonly  	& [200, 400] 	& 0.5 	& 0.88 	& 9.297 	& 5560.0 \\
manifestonly  	& [300, 200] 	& 0.3 	& 0.981 	& 7.589 	& 5560.0 \\
manifestonly  	& [300, 200] 	& 0.4 	& 0.975 	& 8.023 	& 5560.0 \\
manifestonly  	& [300, 200] 	& 0.5 	& 0.974 	& 7.648 	& 4824.0 \\
manifestonly  	& [400, 200] 	& 0.4 	& 0.998 	& 7.316 	& 5560.0 \\
manifestonly  	& [400, 200] 	& 0.5 	& 0.982 	& 7.049 	& 5560.0 \\
	 	& [100, 200] 	& 0.4 	& 0.749 	& 12.865 	& 5560.0 \\
	 	& [10, 10] 	& 0.3 	& 0.695 	& 13.208 	& 3130.0 \\
	 	& [10, 10] 	& 0.4 	& 0.573 	& 15.398 	& 103.0 \\
	 	& [10, 10] 	& 0.5 	& 0.86 	& 10.981 	& 264.0 \\
	 	& [10, 200] 	& 0.3 	& 0.843 	& 11.863 	& 51.0 \\
	 	& [10, 200] 	& 0.4 	& 0.548 	& 14.262 	& 42.0 \\
	 	& [10, 200] 	& 0.5 	& 0.65 	& 13.883 	& 60.0 \\
	 	& [200, 100] 	& 0.4 	& 0.714 	& 13.118 	& 5560.0 \\
	 	& [200, 100] 	& 0.5 	& 0.73 	& 12.995 	& 5560.0 \\
	 	& [200, 200, 200, 200] 	& 0.4 	& 0.627 	& 14.647 	& 5560.0 \\
	 	& [200, 200, 200] 	& 0.1 	& 0.754 	& 10.501 	& 5560.0 \\
	 	& [200, 200, 200] 	& 0.4 	& 0.713 	& 13.082 	& 5560.0 \\
	 	& [200, 200] 	& 0.1 	& 0.783 	& 10.985 	& 5640.0 \\
	 	& [200, 200] 	& 0.2 	& 0.635 	& 13.425 	& 5560.0 \\
	 	& [200, 200] 	& 0.3 	& 0.631 	& 14.523 	& 5560.0 \\
	 	& [200, 200] 	& 0.4 	& 0.621 	& 14.362 	& 5560.0 \\
	 	& [200, 200] 	& 0.5 	& 0.626 	& 14.995 	& 5560.0 \\
	 	& [200, 300] 	& 0.3 	& 0.71 	& 13.237 	& 5560.0 \\
	 	& [200, 300] 	& 0.4 	& 0.619 	& 14.185 	& 5560.0 \\
	 	& [200] 	& 0.4 	& 0.819 	& 11.519 	& 5560.0 \\
	 	& [200] 	& 0.5 	& 0.794 	& 11.919 	& 5560.0 \\
	 	& [300, 200] 	& 0.2 	& 0.7 	& 13.622 	& 5560.0 \\
	 	& [300, 200] 	& 0.4 	& 0.635 	& 14.012 	& 5560.0 \\
	 	& [50, 200] 	& 0.3 	& 0.744 	& 12.349 	& 43.0 \\
	 	& [50, 50] 	& 0.3 	& 0.613 	& 15.45 	& 2403.0 \\
	 	& [50, 50] 	& 0.4 	& 0.593 	& 13.648 	& 54.0 \\
	 	& [50, 50] 	& 0.5 	& 0.51 	& 17.412 	& 51.0 \\
onlyfreq 1  	& [200, 200] 	& 0.3 	& 0.751 	& 13.491 	& 2262.0 \\
onlyfreq 1  	& [200, 200] 	& 0.4 	& 0.532 	& 16.156 	& 5560.0 \\
onlyfreq 1  	& [200, 200] 	& 0.5 	& 0.827 	& 11.494 	& 1069.0 \\
onlyfreq 2  	& [200, 200] 	& 0.3 	& 0.663 	& 14.345 	& 11115.0 \\
onlyfreq 2  	& [200, 200] 	& 0.4 	& 0.678 	& 14.081 	& 5560.0 \\
onlyfreq 2  	& [200, 200] 	& 0.5 	& 0.577 	& 15.122 	& 1084.0 \\
onlyfreq 3  	& [200, 200] 	& 0.3 	& 0.766 	& 13.16 	& 11001.0 \\
onlyfreq 3  	& [200, 200] 	& 0.4 	& 0.652 	& 14.242 	& 5560.0 \\
onlyfreq 4  	& [200, 200] 	& 0.3 	& 0.644 	& 15.445 	& 5560.0 \\
onlyfreq 4  	& [200, 200] 	& 0.4 	& 0.702 	& 13.66 	& 5560.0 \\
onlysmall 1  	& [200, 200] 	& 0.3 	& 0.844 	& 11.411 	& 3056.0 \\
onlysmall 1  	& [200, 200] 	& 0.4 	& 0.838 	& 12.395 	& 5560.0 \\
onlysmall 1  	& [200, 200] 	& 0.5 	& 0.852 	& 11.732 	& 1801.0 \\
onlysmall 2  	& [200, 200] 	& 0.3 	& 0.824 	& 10.817 	& 5560.0 \\
onlysmall 2  	& [200, 200] 	& 0.4 	& 0.748 	& 12.244 	& 5560.0 \\
onlysmall 2  	& [200, 200] 	& 0.5 	& 0.672 	& 13.474 	& 5560.0 \\
onlysmall 3  	& [200, 200] 	& 0.3 	& 0.891 	& 9.829 	& 5560.0 \\
onlysmall 3  	& [200, 200] 	& 0.5 	& 0.745 	& 13.339 	& 5560.0 \\
onlysmall 4  	& [200, 200] 	& 0.4 	& 0.825 	& 11.306 	& 5560.0 \\
onlysmall 5  	& [200, 200] 	& 0.4 	& 0.838 	& 11.966 	& 5560.0 
\end{tabular}
\caption{Missclassification rates achieved for different architectures and feature reductions.}\label{table:feature_reduction}
\end{table*}
%50  100:102  150:159 250:269  500:627  1000:1393  1500:3280  1750:5701

